CRUXEval-X: A Benchmark for Multilingual Code Reasoning, Understanding and Execution

Code benchmarks such as HumanEval are widely adopted to evaluate Large Language Models' (LLMs) coding capabilities. However, there is an unignorable programming language bias in existing code benchmarks -- over 95% code generation benchmarks are dominated by Python, leaving the LLMs' capabilities in other programming languages such as Java and C/C++ unknown. Moreover, coding task bias is also crucial. Most benchmarks focus on code generation capability, while benchmarks for code reasoning (given input, reasoning output; and given output, reasoning input), an essential coding capability, are insufficient. Yet, constructing multi-lingual benchmarks can be expensive and labor-intensive, and codes in contest websites such as Leetcode suffer from data contamination during training. To fill this gap, we propose CRUXEVAL-X, a multi-lingual code reasoning benchmark that contains 19 programming languages. It comprises at least 600 subjects for each language, along with 19K content-consistent tests in total. In particular, the construction pipeline of CRUXEVAL-X works in a fully automated and test-guided manner, which iteratively generates and repairs based on execution feedback. Also, to cross language barriers (e.g., dynamic/static type systems in Python/C++), we formulated various transition rules between language pairs to facilitate translation. Our intensive evaluation of 24 representative LLMs reveals the correlation between language pairs. For example, TypeScript and JavaScript show a significant positive correlation, while Racket has less correlation with other languages. More interestingly, even a model trained solely on Python can achieve at most 34.4% Pass@1 in other languages, revealing the cross-language generalization of LLMs.

==> table/exp.tex <==
\begin{table*}[htbp]
  \centering
  \small
  \setlength{\tabcolsep}{0.85mm}
  \caption{Add caption}
    \begin{tabular}{l|c|ccccccccccccccccccc}
    \toprule
    \multicolumn{21}{c}{\textbf{CRUXEVAL-I Performence}} \\
    \midrule
    \textbf{Models} & \textbf{Size} & \multicolumn{1}{c}{\textbf{cs}} & \multicolumn{1}{c}{\textbf{cpp}} & \multicolumn{1}{c}{\textbf{d}} & \multicolumn{1}{c}{\textbf{go}} & \multicolumn{1}{c}{\textbf{java}} & \multicolumn{1}{c}{\textbf{js}} & \multicolumn{1}{c}{\textbf{jl}} & \multicolumn{1}{c}{\textbf{lua}} & \multicolumn{1}{c}{\textbf{pl}} & \multicolumn{1}{c}{\textbf{php}} & \multicolumn{1}{c}{\textbf{py}} & \multicolumn{1}{c}{\textbf{r}} & \multicolumn{1}{c}{\textbf{rkt}} & \multicolumn{1}{c}{\textbf{rb}} & \multicolumn{1}{c}{\textbf{rs}} & \multicolumn{1}{c}{\textbf{scala}} & \multicolumn{1}{c}{\textbf{sh}} & \multicolumn{1}{c}{\textbf{swift}} & \multicolumn{1}{c}{\textbf{ts}} \\
    \midrule
    GPT-4o & -     & \cellcolor[rgb]{ .557,  .686,  .851} 70.2 & \cellcolor[rgb]{ .592,  .71,  .863} 64.6 & \cellcolor[rgb]{ .549,  .678,  .847} 71.6 & \cellcolor[rgb]{ .525,  .663,  .839} 75.4 & \cellcolor[rgb]{ .561,  .686,  .851} 69.8 & \cellcolor[rgb]{ .541,  .675,  .843} 73.2 & \cellcolor[rgb]{ .58,  .702,  .855} 67.0 & \cellcolor[rgb]{ .541,  .675,  .843} 73.0 & \cellcolor[rgb]{ .557,  .686,  .851} 70.2 & \cellcolor[rgb]{ .529,  .667,  .839} 74.8 & \cellcolor[rgb]{ .557,  .686,  .847} 70.6 & \cellcolor[rgb]{ .533,  .667,  .839} 74.4 & \cellcolor[rgb]{ .576,  .698,  .855} 67.4 & \cellcolor[rgb]{ .549,  .678,  .847} 72.0 & \cellcolor[rgb]{ .537,  .671,  .843} 73.6 & \cellcolor[rgb]{ .588,  .71,  .859} 65.4 & \cellcolor[rgb]{ .557,  .686,  .847} 70.6 & \cellcolor[rgb]{ .533,  .667,  .839} 74.2 & \cellcolor[rgb]{ .533,  .671,  .839} 74.0 \\
    GPT-4o-mini & -     & \cellcolor[rgb]{ .631,  .737,  .875} 58.8 & \cellcolor[rgb]{ .675,  .769,  .89} 52.2 & \cellcolor[rgb]{ .62,  .729,  .871} 60.6 & \cellcolor[rgb]{ .612,  .722,  .867} 62.0 & \cellcolor[rgb]{ .639,  .745,  .878} 57.2 & \cellcolor[rgb]{ .627,  .733,  .875} 59.6 & \cellcolor[rgb]{ .647,  .749,  .878} 56.2 & \cellcolor[rgb]{ .6,  .718,  .863} 63.4 & \cellcolor[rgb]{ .639,  .745,  .878} 57.4 & \cellcolor[rgb]{ .616,  .729,  .871} 61.0 & \cellcolor[rgb]{ .627,  .733,  .875} 59.6 & \cellcolor[rgb]{ .62,  .729,  .871} 60.4 & \cellcolor[rgb]{ .678,  .773,  .89} 51.2 & \cellcolor[rgb]{ .612,  .725,  .867} 61.6 & \cellcolor[rgb]{ .616,  .725,  .871} 61.2 & \cellcolor[rgb]{ .671,  .765,  .886} 52.6 & \cellcolor[rgb]{ .639,  .745,  .878} 57.2 & \cellcolor[rgb]{ .6,  .718,  .863} 63.4 & \cellcolor[rgb]{ .616,  .725,  .871} 61.2 \\
    GPT-3.5 Turbo & -     & \cellcolor[rgb]{ .675,  .769,  .89} 52.2 & \cellcolor[rgb]{ .757,  .827,  .918} 39.2 & \cellcolor[rgb]{ .686,  .776,  .894} 50.2 & \cellcolor[rgb]{ .667,  .761,  .886} 53.4 & \cellcolor[rgb]{ .651,  .753,  .882} 55.4 & \cellcolor[rgb]{ .686,  .776,  .894} 50.0 & \cellcolor[rgb]{ .706,  .792,  .898} 47.0 & \cellcolor[rgb]{ .667,  .765,  .886} 53.2 & \cellcolor[rgb]{ .702,  .788,  .898} 47.6 & \cellcolor[rgb]{ .675,  .769,  .89} 52.2 & \cellcolor[rgb]{ .675,  .769,  .89} 51.6 & \cellcolor[rgb]{ .694,  .784,  .898} 48.6 & \cellcolor[rgb]{ .718,  .8,  .902} 45.4 & \cellcolor[rgb]{ .69,  .78,  .894} 49.6 & \cellcolor[rgb]{ .667,  .765,  .886} 53.0 & \cellcolor[rgb]{ .659,  .757,  .886} 54.2 & \cellcolor[rgb]{ .702,  .788,  .898} 47.6 & \cellcolor[rgb]{ .635,  .741,  .875} 58.2 & \cellcolor[rgb]{ .698,  .784,  .898} 48.4 \\
    Deepseekcoder-V2 & 236B  & \cellcolor[rgb]{ .6,  .714,  .863} 63.8 & \cellcolor[rgb]{ .643,  .745,  .878} 57.0 & \cellcolor[rgb]{ .58,  .702,  .859} 66.6 & \cellcolor[rgb]{ .596,  .714,  .863} 64.0 & \cellcolor[rgb]{ .592,  .71,  .863} 64.8 & \cellcolor[rgb]{ .58,  .702,  .855} 67.0 & \cellcolor[rgb]{ .635,  .741,  .875} 58.4 & \cellcolor[rgb]{ .612,  .722,  .867} 62.0 & \cellcolor[rgb]{ .616,  .725,  .871} 61.4 & \cellcolor[rgb]{ .596,  .714,  .863} 64.2 & \cellcolor[rgb]{ .596,  .714,  .863} 64.0 & \cellcolor[rgb]{ .588,  .706,  .859} 65.8 & \cellcolor[rgb]{ .635,  .741,  .875} 58.0 & \cellcolor[rgb]{ .604,  .718,  .867} 63.2 & \cellcolor[rgb]{ .6,  .718,  .863} 63.6 & \cellcolor[rgb]{ .635,  .741,  .875} 58.2 & \cellcolor[rgb]{ .608,  .722,  .867} 62.4 & \cellcolor[rgb]{ .608,  .722,  .867} 62.6 & \cellcolor[rgb]{ .58,  .702,  .859} 66.6 \\
    Qwen2-Instruct & 72B   & \cellcolor[rgb]{ .675,  .769,  .89} 52.0 & \cellcolor[rgb]{ .659,  .757,  .886} 54.2 & \cellcolor[rgb]{ .69,  .78,  .894} 49.6 & \cellcolor[rgb]{ .651,  .753,  .882} 55.4 & \cellcolor[rgb]{ .686,  .776,  .894} 50.0 & \cellcolor[rgb]{ .675,  .769,  .89} 51.6 & \cellcolor[rgb]{ .678,  .773,  .89} 51.0 & \cellcolor[rgb]{ .678,  .773,  .89} 51.2 & \cellcolor[rgb]{ .702,  .788,  .898} 47.8 & \cellcolor[rgb]{ .655,  .753,  .882} 55.2 & \cellcolor[rgb]{ .671,  .765,  .886} 52.4 & \cellcolor[rgb]{ .667,  .765,  .886} 53.2 & \cellcolor[rgb]{ .702,  .788,  .898} 47.8 & \cellcolor[rgb]{ .659,  .757,  .882} 54.4 & \cellcolor[rgb]{ .639,  .745,  .878} 57.2 & \cellcolor[rgb]{ .682,  .776,  .894} 50.6 & \cellcolor[rgb]{ .671,  .765,  .886} 52.4 & \cellcolor[rgb]{ .675,  .769,  .89} 51.6 & \cellcolor[rgb]{ .675,  .769,  .89} 52.0 \\
    CodeLlama-Python & 34B   & \cellcolor[rgb]{ .757,  .827,  .918} 38.8 & \cellcolor[rgb]{ .749,  .824,  .914} 40.0 & \cellcolor[rgb]{ .757,  .827,  .918} 39.2 & \cellcolor[rgb]{ .757,  .827,  .918} 39.0 & \cellcolor[rgb]{ .741,  .816,  .914} 41.4 & \cellcolor[rgb]{ .714,  .796,  .902} 45.8 & \cellcolor[rgb]{ .718,  .8,  .906} 44.8 & \cellcolor[rgb]{ .718,  .8,  .906} 45.0 & \cellcolor[rgb]{ .729,  .808,  .91} 43.2 & \cellcolor[rgb]{ .698,  .788,  .898} 48.0 & \cellcolor[rgb]{ .706,  .792,  .902} 46.8 & \cellcolor[rgb]{ .737,  .812,  .91} 42.2 & \cellcolor[rgb]{ .757,  .827,  .918} 38.8 & \cellcolor[rgb]{ .725,  .804,  .906} 44.0 & \cellcolor[rgb]{ .722,  .804,  .906} 44.2 & \cellcolor[rgb]{ .729,  .808,  .91} 43.0 & \cellcolor[rgb]{ .722,  .8,  .906} 44.6 & \cellcolor[rgb]{ .718,  .8,  .906} 45.0 & \cellcolor[rgb]{ .725,  .804,  .906} 44.0 \\
    CodeLlama-Instruct & 34B   & \cellcolor[rgb]{ .722,  .8,  .906} 44.6 & \cellcolor[rgb]{ .698,  .784,  .898} 48.4 & \cellcolor[rgb]{ .725,  .804,  .906} 43.8 & \cellcolor[rgb]{ .714,  .796,  .902} 46.0 & \cellcolor[rgb]{ .722,  .804,  .906} 44.4 & \cellcolor[rgb]{ .671,  .765,  .886} 52.6 & \cellcolor[rgb]{ .682,  .776,  .894} 50.4 & \cellcolor[rgb]{ .69,  .78,  .894} 49.4 & \cellcolor[rgb]{ .714,  .796,  .902} 46.0 & \cellcolor[rgb]{ .675,  .769,  .89} 52.0 & \cellcolor[rgb]{ .678,  .773,  .89} 51.2 & \cellcolor[rgb]{ .698,  .784,  .898} 48.4 & \cellcolor[rgb]{ .733,  .812,  .91} 42.4 & \cellcolor[rgb]{ .698,  .784,  .898} 48.2 & \cellcolor[rgb]{ .694,  .784,  .898} 48.6 & \cellcolor[rgb]{ .698,  .788,  .898} 48.0 & \cellcolor[rgb]{ .71,  .796,  .902} 46.2 & \cellcolor[rgb]{ .69,  .78,  .894} 49.4 & \cellcolor[rgb]{ .667,  .765,  .886} 53.2 \\
    CodeLlama & 34B   & \cellcolor[rgb]{ .749,  .82,  .914} 40.4 & \cellcolor[rgb]{ .722,  .8,  .906} 44.6 & \cellcolor[rgb]{ .714,  .796,  .902} 45.6 & \cellcolor[rgb]{ .741,  .816,  .914} 41.2 & \cellcolor[rgb]{ .757,  .827,  .918} 39.0 & \cellcolor[rgb]{ .686,  .776,  .894} 50.0 & \cellcolor[rgb]{ .694,  .78,  .894} 49.0 & \cellcolor[rgb]{ .706,  .792,  .898} 47.0 & \cellcolor[rgb]{ .71,  .792,  .902} 46.6 & \cellcolor[rgb]{ .694,  .784,  .898} 48.8 & \cellcolor[rgb]{ .686,  .776,  .894} 49.8 & \cellcolor[rgb]{ .702,  .788,  .898} 47.6 & \cellcolor[rgb]{ .753,  .824,  .918} 39.8 & \cellcolor[rgb]{ .71,  .792,  .902} 46.6 & \cellcolor[rgb]{ .706,  .792,  .902} 46.8 & \cellcolor[rgb]{ .722,  .8,  .906} 44.6 & \cellcolor[rgb]{ .722,  .804,  .906} 44.4 & \cellcolor[rgb]{ .686,  .776,  .894} 50.0 & \cellcolor[rgb]{ .694,  .784,  .898} 48.6 \\
    WizardCoder-V1.1 & 33B   & \cellcolor[rgb]{ .718,  .8,  .906} 44.8 & \cellcolor[rgb]{ .843,  .89,  .949} 25.4 & \cellcolor[rgb]{ .71,  .792,  .902} 46.4 & \cellcolor[rgb]{ .702,  .788,  .898} 47.6 & \cellcolor[rgb]{ .698,  .784,  .898} 48.4 & \cellcolor[rgb]{ .714,  .796,  .902} 45.6 & \cellcolor[rgb]{ .69,  .78,  .894} 49.2 & \cellcolor[rgb]{ .694,  .784,  .898} 48.8 & \cellcolor[rgb]{ .722,  .8,  .906} 44.6 & \cellcolor[rgb]{ .686,  .776,  .894} 50.0 & \cellcolor[rgb]{ .686,  .776,  .894} 50.0 & \cellcolor[rgb]{ .718,  .8,  .906} 45.0 & \cellcolor[rgb]{ .733,  .812,  .91} 42.4 & \cellcolor[rgb]{ .69,  .78,  .894} 49.2 & \cellcolor[rgb]{ .698,  .784,  .898} 48.2 & \cellcolor[rgb]{ .698,  .784,  .898} 48.2 & \cellcolor[rgb]{ .718,  .8,  .902} 45.4 & \cellcolor[rgb]{ .678,  .773,  .89} 51.0 & \cellcolor[rgb]{ .71,  .792,  .902} 46.4 \\
    Deepseekcoder-instruct & 33B   & \cellcolor[rgb]{ .714,  .796,  .902} 46.0 & \cellcolor[rgb]{ .725,  .808,  .906} 43.6 & \cellcolor[rgb]{ .686,  .776,  .894} 49.8 & \cellcolor[rgb]{ .694,  .78,  .894} 49.0 & \cellcolor[rgb]{ .706,  .792,  .902} 46.8 & \cellcolor[rgb]{ .694,  .784,  .898} 48.8 & \cellcolor[rgb]{ .706,  .792,  .898} 47.0 & \cellcolor[rgb]{ .686,  .776,  .894} 50.0 & \cellcolor[rgb]{ .706,  .792,  .902} 46.8 & \cellcolor[rgb]{ .675,  .769,  .89} 52.0 & \cellcolor[rgb]{ .675,  .769,  .89} 51.8 & \cellcolor[rgb]{ .698,  .784,  .898} 48.2 & \cellcolor[rgb]{ .741,  .816,  .914} 41.6 & \cellcolor[rgb]{ .675,  .769,  .89} 52.0 & \cellcolor[rgb]{ .698,  .784,  .898} 48.4 & \cellcolor[rgb]{ .706,  .792,  .898} 47.0 & \cellcolor[rgb]{ .698,  .784,  .898} 48.2 & \cellcolor[rgb]{ .675,  .769,  .89} 52.2 & \cellcolor[rgb]{ .69,  .78,  .894} 49.6 \\
    Deepseekcoder-base & 33B   & \cellcolor[rgb]{ .741,  .816,  .914} 41.2 & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 & \cellcolor[rgb]{ .729,  .808,  .91} 43.2 & \cellcolor[rgb]{ .714,  .796,  .902} 45.6 & \cellcolor[rgb]{ .725,  .804,  .906} 43.8 & \cellcolor[rgb]{ .714,  .796,  .902} 46.0 & \cellcolor[rgb]{ .702,  .788,  .898} 47.6 & \cellcolor[rgb]{ .702,  .788,  .898} 47.4 & \cellcolor[rgb]{ .706,  .788,  .898} 47.2 & \cellcolor[rgb]{ .694,  .784,  .898} 48.6 & \cellcolor[rgb]{ .69,  .78,  .894} 49.2 & \cellcolor[rgb]{ .682,  .776,  .894} 50.6 & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 & \cellcolor[rgb]{ .702,  .788,  .898} 47.4 & \cellcolor[rgb]{ .706,  .792,  .902} 46.8 & \cellcolor[rgb]{ .725,  .804,  .906} 44.0 & \cellcolor[rgb]{ .71,  .792,  .902} 46.4 & \cellcolor[rgb]{ .698,  .784,  .898} 48.2 & \cellcolor[rgb]{ .718,  .8,  .906} 45.0 \\
    Starcoder2 & 15B   & \cellcolor[rgb]{ .741,  .816,  .914} 41.4 & \cellcolor[rgb]{ .725,  .804,  .906} 43.8 & \cellcolor[rgb]{ .675,  .769,  .89} 51.6 & \cellcolor[rgb]{ .718,  .8,  .906} 45.2 & \cellcolor[rgb]{ .733,  .812,  .91} 42.6 & \cellcolor[rgb]{ .725,  .804,  .906} 44.0 & \cellcolor[rgb]{ .698,  .784,  .898} 48.2 & \cellcolor[rgb]{ .722,  .8,  .906} 44.6 & \cellcolor[rgb]{ .718,  .8,  .906} 44.8 & \cellcolor[rgb]{ .686,  .776,  .894} 49.8 & \cellcolor[rgb]{ .71,  .792,  .902} 46.6 & \cellcolor[rgb]{ .714,  .796,  .902} 45.8 & \cellcolor[rgb]{ .718,  .8,  .906} 45.0 & \cellcolor[rgb]{ .694,  .78,  .894} 49.0 & \cellcolor[rgb]{ .71,  .792,  .902} 46.6 & \cellcolor[rgb]{ .769,  .835,  .922} 37.0 & \cellcolor[rgb]{ .702,  .788,  .898} 47.4 & \cellcolor[rgb]{ .675,  .769,  .89} 52.2 & \cellcolor[rgb]{ .71,  .796,  .902} 46.2 \\
    WizardCoder-V1.0 & 15B   & \cellcolor[rgb]{ .82,  .871,  .937} 29.2 & \cellcolor[rgb]{ .812,  .867,  .937} 30.0 & \cellcolor[rgb]{ .808,  .867,  .937} 30.6 & \cellcolor[rgb]{ .824,  .875,  .941} 28.6 & \cellcolor[rgb]{ .816,  .871,  .937} 29.6 & \cellcolor[rgb]{ .796,  .855,  .929} 33.0 & \cellcolor[rgb]{ .784,  .847,  .925} 34.8 & \cellcolor[rgb]{ .792,  .851,  .929} 33.6 & \cellcolor[rgb]{ .773,  .839,  .922} 36.2 & \cellcolor[rgb]{ .769,  .835,  .922} 36.8 & \cellcolor[rgb]{ .792,  .855,  .929} 33.2 & \cellcolor[rgb]{ .792,  .851,  .929} 33.4 & \cellcolor[rgb]{ .773,  .839,  .922} 36.4 & \cellcolor[rgb]{ .792,  .851,  .929} 33.6 & \cellcolor[rgb]{ .796,  .855,  .929} 33.0 & \cellcolor[rgb]{ .82,  .871,  .937} 29.0 & \cellcolor[rgb]{ .78,  .843,  .925} 35.0 & \cellcolor[rgb]{ .788,  .851,  .929} 34.0 & \cellcolor[rgb]{ .796,  .855,  .933} 32.4 \\
    Starcoder & 15B   & \cellcolor[rgb]{ .824,  .875,  .941} 28.2 & \cellcolor[rgb]{ .812,  .867,  .937} 30.0 & \cellcolor[rgb]{ .796,  .855,  .929} 33.0 & \cellcolor[rgb]{ .792,  .855,  .929} 33.2 & \cellcolor[rgb]{ .792,  .851,  .929} 33.4 & \cellcolor[rgb]{ .78,  .843,  .925} 35.2 & \cellcolor[rgb]{ .784,  .847,  .929} 34.4 & \cellcolor[rgb]{ .804,  .859,  .933} 31.6 & \cellcolor[rgb]{ .788,  .851,  .929} 34.0 & \cellcolor[rgb]{ .773,  .839,  .922} 36.4 & \cellcolor[rgb]{ .784,  .847,  .925} 34.8 & \cellcolor[rgb]{ .792,  .851,  .929} 33.4 & \cellcolor[rgb]{ .773,  .839,  .922} 36.6 & \cellcolor[rgb]{ .78,  .843,  .925} 35.0 & \cellcolor[rgb]{ .784,  .847,  .925} 34.8 & \cellcolor[rgb]{ .831,  .878,  .941} 27.4 & \cellcolor[rgb]{ .769,  .835,  .922} 37.0 & \cellcolor[rgb]{ .808,  .863,  .933} 30.8 & \cellcolor[rgb]{ .792,  .855,  .929} 33.2 \\
    phi-3-instruct & 14B   & \cellcolor[rgb]{ .8,  .859,  .933} 31.8 & \cellcolor[rgb]{ .839,  .886,  .945} 26.0 & \cellcolor[rgb]{ .757,  .827,  .918} 38.8 & \cellcolor[rgb]{ .773,  .839,  .922} 36.4 & \cellcolor[rgb]{ .769,  .835,  .922} 37.2 & \cellcolor[rgb]{ .733,  .812,  .91} 42.4 & \cellcolor[rgb]{ .773,  .839,  .922} 36.2 & \cellcolor[rgb]{ .769,  .835,  .922} 37.2 & \cellcolor[rgb]{ .776,  .843,  .925} 35.6 & \cellcolor[rgb]{ .741,  .816,  .914} 41.2 & \cellcolor[rgb]{ .729,  .808,  .91} 43.4 & \cellcolor[rgb]{ .757,  .827,  .918} 39.2 & \cellcolor[rgb]{ .847,  .894,  .949} 24.4 & \cellcolor[rgb]{ .776,  .839,  .925} 36.0 & \cellcolor[rgb]{ .769,  .835,  .922} 36.8 & \cellcolor[rgb]{ .761,  .831,  .922} 38.0 & \cellcolor[rgb]{ .792,  .851,  .929} 33.6 & \cellcolor[rgb]{ .741,  .816,  .914} 41.2 & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 \\
    Llama-3-Instruct & 8B    & \cellcolor[rgb]{ .769,  .835,  .922} 37.0 & \cellcolor[rgb]{ .773,  .839,  .922} 36.4 & \cellcolor[rgb]{ .78,  .843,  .925} 35.0 & \cellcolor[rgb]{ .757,  .827,  .918} 38.6 & \cellcolor[rgb]{ .773,  .839,  .922} 36.2 & \cellcolor[rgb]{ .761,  .831,  .918} 38.4 & \cellcolor[rgb]{ .753,  .824,  .918} 39.6 & \cellcolor[rgb]{ .749,  .824,  .914} 40.0 & \cellcolor[rgb]{ .773,  .839,  .922} 36.2 & \cellcolor[rgb]{ .773,  .839,  .922} 36.6 & \cellcolor[rgb]{ .761,  .831,  .918} 38.4 & \cellcolor[rgb]{ .737,  .812,  .91} 42.2 & \cellcolor[rgb]{ .851,  .894,  .949} 24.2 & \cellcolor[rgb]{ .776,  .843,  .925} 35.8 & \cellcolor[rgb]{ .765,  .831,  .922} 37.6 & \cellcolor[rgb]{ .761,  .831,  .922} 38.0 & \cellcolor[rgb]{ .804,  .859,  .933} 31.6 & \cellcolor[rgb]{ .737,  .812,  .91} 42.2 & \cellcolor[rgb]{ .761,  .831,  .918} 38.2 \\
    CodeQwen1.5-Chat & 7B    & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 & \cellcolor[rgb]{ .737,  .812,  .91} 42.0 & \cellcolor[rgb]{ .729,  .808,  .91} 43.0 & \cellcolor[rgb]{ .71,  .792,  .902} 46.4 & \cellcolor[rgb]{ .722,  .8,  .906} 44.6 & \cellcolor[rgb]{ .725,  .804,  .906} 43.8 & \cellcolor[rgb]{ .737,  .812,  .91} 42.2 & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 & \cellcolor[rgb]{ .741,  .816,  .914} 41.6 & \cellcolor[rgb]{ .718,  .8,  .906} 44.8 & \cellcolor[rgb]{ .729,  .808,  .91} 43.0 & \cellcolor[rgb]{ .729,  .808,  .91} 43.4 & \cellcolor[rgb]{ .761,  .831,  .918} 38.2 & \cellcolor[rgb]{ .725,  .808,  .906} 43.6 & \cellcolor[rgb]{ .737,  .812,  .91} 42.0 & \cellcolor[rgb]{ .753,  .824,  .918} 39.4 & \cellcolor[rgb]{ .71,  .792,  .902} 46.6 & \cellcolor[rgb]{ .714,  .796,  .902} 45.8 & \cellcolor[rgb]{ .725,  .808,  .906} 43.6 \\
    CodeLlama-Instruct & 7B    & \cellcolor[rgb]{ .757,  .827,  .918} 38.6 & \cellcolor[rgb]{ .776,  .839,  .925} 36.0 & \cellcolor[rgb]{ .761,  .831,  .918} 38.4 & \cellcolor[rgb]{ .761,  .831,  .918} 38.4 & \cellcolor[rgb]{ .761,  .831,  .918} 38.2 & \cellcolor[rgb]{ .753,  .824,  .918} 39.6 & \cellcolor[rgb]{ .737,  .812,  .91} 42.2 & \cellcolor[rgb]{ .729,  .808,  .91} 43.4 & \cellcolor[rgb]{ .773,  .839,  .922} 36.4 & \cellcolor[rgb]{ .749,  .82,  .914} 40.4 & \cellcolor[rgb]{ .745,  .82,  .914} 41.0 & \cellcolor[rgb]{ .745,  .82,  .914} 41.0 & \cellcolor[rgb]{ .757,  .827,  .918} 38.8 & \cellcolor[rgb]{ .741,  .816,  .914} 41.6 & \cellcolor[rgb]{ .765,  .831,  .922} 37.6 & \cellcolor[rgb]{ .733,  .812,  .91} 42.6 & \cellcolor[rgb]{ .753,  .824,  .918} 39.6 & \cellcolor[rgb]{ .749,  .824,  .914} 40.2 & \cellcolor[rgb]{ .745,  .82,  .914} 41.0 \\
    CodeLlama-hf & 7B    & \cellcolor[rgb]{ .773,  .839,  .922} 36.4 & \cellcolor[rgb]{ .773,  .839,  .922} 36.2 & \cellcolor[rgb]{ .769,  .835,  .922} 36.8 & \cellcolor[rgb]{ .784,  .847,  .925} 34.6 & \cellcolor[rgb]{ .773,  .839,  .922} 36.4 & \cellcolor[rgb]{ .773,  .839,  .922} 36.6 & \cellcolor[rgb]{ .749,  .824,  .914} 40.2 & \cellcolor[rgb]{ .753,  .824,  .918} 39.6 & \cellcolor[rgb]{ .776,  .839,  .925} 36.0 & \cellcolor[rgb]{ .753,  .824,  .918} 39.4 & \cellcolor[rgb]{ .749,  .824,  .914} 40.2 & \cellcolor[rgb]{ .749,  .824,  .914} 40.0 & \cellcolor[rgb]{ .773,  .839,  .922} 36.6 & \cellcolor[rgb]{ .757,  .827,  .918} 39.2 & \cellcolor[rgb]{ .78,  .843,  .925} 35.4 & \cellcolor[rgb]{ .765,  .831,  .922} 37.8 & \cellcolor[rgb]{ .769,  .835,  .922} 36.8 & \cellcolor[rgb]{ .757,  .827,  .918} 39.2 & \cellcolor[rgb]{ .757,  .827,  .918} 38.8 \\
    Deepseekcoder-instruct & 6.7B  & \cellcolor[rgb]{ .78,  .843,  .925} 35.0 & \cellcolor[rgb]{ .769,  .835,  .922} 37.0 & \cellcolor[rgb]{ .776,  .843,  .925} 35.6 & \cellcolor[rgb]{ .749,  .82,  .914} 40.4 & \cellcolor[rgb]{ .78,  .843,  .925} 35.0 & \cellcolor[rgb]{ .773,  .839,  .922} 36.6 & \cellcolor[rgb]{ .757,  .827,  .918} 39.2 & \cellcolor[rgb]{ .757,  .827,  .918} 38.8 & \cellcolor[rgb]{ .753,  .824,  .918} 39.4 & \cellcolor[rgb]{ .737,  .812,  .91} 42.2 & \cellcolor[rgb]{ .761,  .831,  .918} 38.2 & \cellcolor[rgb]{ .737,  .812,  .91} 42.0 & \cellcolor[rgb]{ .769,  .835,  .922} 37.2 & \cellcolor[rgb]{ .749,  .824,  .914} 40.2 & \cellcolor[rgb]{ .765,  .835,  .922} 37.4 & \cellcolor[rgb]{ .769,  .835,  .922} 36.8 & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 & \cellcolor[rgb]{ .745,  .82,  .914} 40.8 & \cellcolor[rgb]{ .788,  .847,  .929} 34.2 \\
    Deepseekcoder-base & 6.7B  & \cellcolor[rgb]{ .757,  .827,  .918} 38.8 & \cellcolor[rgb]{ .733,  .812,  .91} 42.4 & \cellcolor[rgb]{ .741,  .816,  .914} 41.2 & \cellcolor[rgb]{ .729,  .808,  .91} 43.2 & \cellcolor[rgb]{ .749,  .82,  .914} 40.4 & \cellcolor[rgb]{ .725,  .808,  .906} 43.6 & \cellcolor[rgb]{ .733,  .812,  .91} 42.6 & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 & \cellcolor[rgb]{ .741,  .816,  .914} 41.6 & \cellcolor[rgb]{ .71,  .792,  .902} 46.4 & \cellcolor[rgb]{ .741,  .816,  .914} 41.4 & \cellcolor[rgb]{ .71,  .796,  .902} 46.2 & \cellcolor[rgb]{ .729,  .808,  .91} 43.0 & \cellcolor[rgb]{ .722,  .8,  .906} 44.6 & \cellcolor[rgb]{ .741,  .816,  .914} 41.6 & \cellcolor[rgb]{ .745,  .82,  .914} 40.8 & \cellcolor[rgb]{ .718,  .8,  .906} 44.8 & \cellcolor[rgb]{ .729,  .808,  .91} 43.4 & \cellcolor[rgb]{ .737,  .816,  .91} 41.8 \\
    CodeGen-multi & 6B    & \cellcolor[rgb]{ .82,  .875,  .941} 28.8 & \cellcolor[rgb]{ .843,  .89,  .949} 25.4 & \cellcolor[rgb]{ .965,  .976,  .988} 6.2 & \cellcolor[rgb]{ .839,  .886,  .945} 25.6 & \cellcolor[rgb]{ .773,  .839,  .922} 36.2 & \cellcolor[rgb]{ .843,  .89,  .949} 25.2 & \cellcolor[rgb]{ .894,  .925,  .965} 17.4 & \cellcolor[rgb]{ .847,  .894,  .949} 24.4 & \cellcolor[rgb]{ .761,  .831,  .918} 38.4 & \cellcolor[rgb]{ .859,  .902,  .953} 22.8 & \cellcolor[rgb]{ .859,  .902,  .953} 22.6 & \cellcolor[rgb]{ .831,  .878,  .945} 27.2 & \cellcolor[rgb]{ .902,  .929,  .969} 16.2 & \cellcolor[rgb]{ .961,  .973,  .988} 6.4 & \cellcolor[rgb]{ .882,  .918,  .961} 18.8 & \cellcolor[rgb]{ .808,  .863,  .933} 31.0 & \cellcolor[rgb]{ .694,  .784,  .898} 48.6 & \cellcolor[rgb]{ .796,  .855,  .933} 32.4 & \cellcolor[rgb]{ .843,  .89,  .949} 25.2 \\
    phi-1\_5 & 1.3B  & \cellcolor[rgb]{ .82,  .871,  .937} 29.2 & \cellcolor[rgb]{ .902,  .929,  .969} 16.0 & \cellcolor[rgb]{ .922,  .945,  .973} 13.2 & \cellcolor[rgb]{ .839,  .886,  .945} 25.8 & \cellcolor[rgb]{ .835,  .882,  .945} 26.8 & \cellcolor[rgb]{ .941,  .957,  .98} 9.8 & \cellcolor[rgb]{ .812,  .867,  .937} 30.4 & \cellcolor[rgb]{ .835,  .882,  .945} 26.6 & \cellcolor[rgb]{ .89,  .922,  .965} 17.8 & \cellcolor[rgb]{ .835,  .882,  .945} 26.6 & \cellcolor[rgb]{ .839,  .886,  .945} 25.8 & \cellcolor[rgb]{ .949,  .965,  .984} 8.4 & \cellcolor[rgb]{ .961,  .973,  .988} 6.6 & \cellcolor[rgb]{ .996,  .996,  1} 1.4 & \cellcolor[rgb]{ .843,  .89,  .949} 25.2 & \cellcolor[rgb]{ .812,  .867,  .937} 30.4 & \cellcolor[rgb]{ .784,  .847,  .929} 34.4 & \cellcolor[rgb]{ .835,  .882,  .945} 26.6 & \cellcolor[rgb]{ .808,  .863,  .933} 30.8 \\
    phi-1 & 1.3B  & 0.2   & \cellcolor[rgb]{ .961,  .973,  .988} 7.0 & \cellcolor[rgb]{ .941,  .961,  .98} 9.6 & \cellcolor[rgb]{ .98,  .988,  .996} 3.6 & \cellcolor[rgb]{ .984,  .992,  .996} 2.8 & \cellcolor[rgb]{ .894,  .925,  .965} 17.0 & \cellcolor[rgb]{ .882,  .918,  .961} 19.0 & \cellcolor[rgb]{ .894,  .925,  .965} 17.4 & \cellcolor[rgb]{ .855,  .898,  .949} 23.6 & \cellcolor[rgb]{ .945,  .961,  .98} 9.2 & \cellcolor[rgb]{ .929,  .949,  .976} 11.8 & \cellcolor[rgb]{ .945,  .961,  .98} 9.4 & \cellcolor[rgb]{ .933,  .953,  .976} 11.2 & \cellcolor[rgb]{ .961,  .973,  .988} 6.8 & \cellcolor[rgb]{ .969,  .98,  .992} 5.4 & \cellcolor[rgb]{ .992,  .996,  1} 1.8 & \cellcolor[rgb]{ .878,  .914,  .961} 19.8 & \cellcolor[rgb]{ .914,  .941,  .973} 14.0 & \cellcolor[rgb]{ .914,  .941,  .973} 14.0 \\
    \midrule
    Average &       & 40.4  & 38.3  & 40.8  & 42.4  & 41.7  & 43.1  & 43.1  & 43.9  & 42.5  & 45.0  & 44.1  & 43.2  & 38.0  & 41.7  & 42.7  & 41.1  & 44.3  & 45.4  & 43.8 \\
    \midrule
    \multicolumn{21}{c}{\textbf{CRUXEVAL-O Performence}} \\
    \midrule
    \textbf{Models} & \textbf{Size} & \multicolumn{1}{c}{\textbf{cs}} & \multicolumn{1}{c}{\textbf{cpp}} & \multicolumn{1}{c}{\textbf{d}} & \multicolumn{1}{c}{\textbf{go}} & \multicolumn{1}{c}{\textbf{java}} & \multicolumn{1}{c}{\textbf{js}} & \multicolumn{1}{c}{\textbf{jl}} & \multicolumn{1}{c}{\textbf{lua}} & \multicolumn{1}{c}{\textbf{pl}} & \multicolumn{1}{c}{\textbf{php}} & \multicolumn{1}{c}{\textbf{py}} & \multicolumn{1}{c}{\textbf{r}} & \multicolumn{1}{c}{\textbf{rkt}} & \multicolumn{1}{c}{\textbf{rb}} & \multicolumn{1}{c}{\textbf{rs}} & \multicolumn{1}{c}{\textbf{scala}} & \multicolumn{1}{c}{\textbf{sh}} & \multicolumn{1}{c}{\textbf{swift}} & \multicolumn{1}{c}{\textbf{ts}} \\
    \midrule
    GPT-4o & -     & \cellcolor[rgb]{ .529,  .663,  .839} 75.0 & \cellcolor[rgb]{ .529,  .667,  .839} 74.8 & \cellcolor[rgb]{ .553,  .682,  .847} 71.4 & \cellcolor[rgb]{ .514,  .655,  .835} 77.0 & \cellcolor[rgb]{ .541,  .675,  .843} 73.2 & \cellcolor[rgb]{ .51,  .651,  .831} 77.6 & \cellcolor[rgb]{ .537,  .671,  .843} 73.6 & \cellcolor[rgb]{ .529,  .667,  .839} 74.8 & \cellcolor[rgb]{ .533,  .671,  .839} 74.0 & \cellcolor[rgb]{ .525,  .663,  .839} 75.4 & \cellcolor[rgb]{ .525,  .663,  .839} 75.4 & \cellcolor[rgb]{ .549,  .678,  .847} 72.0 & \cellcolor[rgb]{ .553,  .682,  .847} 70.8 & \cellcolor[rgb]{ .533,  .671,  .839} 74.0 & \cellcolor[rgb]{ .533,  .667,  .839} 74.4 & \cellcolor[rgb]{ .549,  .678,  .847} 71.8 & \cellcolor[rgb]{ .549,  .678,  .847} 71.6 & \cellcolor[rgb]{ .522,  .659,  .835} 76.0 & \cellcolor[rgb]{ .518,  .659,  .835} 76.4 \\
    GPT-4o-mini & -     & \cellcolor[rgb]{ .604,  .718,  .867} 63.0 & \cellcolor[rgb]{ .604,  .718,  .867} 63.0 & \cellcolor[rgb]{ .616,  .725,  .871} 61.4 & \cellcolor[rgb]{ .6,  .718,  .863} 63.4 & \cellcolor[rgb]{ .663,  .761,  .886} 54.0 & \cellcolor[rgb]{ .612,  .725,  .867} 61.8 & \cellcolor[rgb]{ .635,  .741,  .878} 57.8 & \cellcolor[rgb]{ .624,  .733,  .871} 60.0 & \cellcolor[rgb]{ .639,  .745,  .878} 57.4 & \cellcolor[rgb]{ .596,  .714,  .863} 64.2 & \cellcolor[rgb]{ .612,  .725,  .867} 61.6 & \cellcolor[rgb]{ .627,  .733,  .875} 59.6 & \cellcolor[rgb]{ .643,  .749,  .878} 56.6 & \cellcolor[rgb]{ .616,  .725,  .871} 61.2 & \cellcolor[rgb]{ .612,  .725,  .867} 61.8 & \cellcolor[rgb]{ .616,  .725,  .871} 61.2 & \cellcolor[rgb]{ .647,  .749,  .878} 56.2 & \cellcolor[rgb]{ .604,  .718,  .867} 63.0 & \cellcolor[rgb]{ .616,  .725,  .871} 61.2 \\
    GPT-3.5 Turbo & -     & \cellcolor[rgb]{ .659,  .757,  .886} 54.2 & \cellcolor[rgb]{ .729,  .808,  .91} 43.2 & \cellcolor[rgb]{ .647,  .749,  .882} 56.0 & \cellcolor[rgb]{ .667,  .765,  .886} 53.2 & \cellcolor[rgb]{ .725,  .808,  .906} 43.6 & \cellcolor[rgb]{ .647,  .749,  .878} 56.2 & \cellcolor[rgb]{ .659,  .757,  .886} 54.2 & \cellcolor[rgb]{ .659,  .757,  .882} 54.6 & \cellcolor[rgb]{ .675,  .769,  .89} 51.8 & \cellcolor[rgb]{ .655,  .753,  .882} 55.2 & \cellcolor[rgb]{ .639,  .745,  .878} 57.2 & \cellcolor[rgb]{ .69,  .78,  .894} 49.4 & \cellcolor[rgb]{ .698,  .788,  .898} 48.0 & \cellcolor[rgb]{ .647,  .749,  .878} 56.4 & \cellcolor[rgb]{ .659,  .757,  .882} 54.6 & \cellcolor[rgb]{ .647,  .749,  .878} 56.4 & \cellcolor[rgb]{ .678,  .773,  .89} 51.0 & \cellcolor[rgb]{ .635,  .741,  .878} 57.8 & \cellcolor[rgb]{ .663,  .761,  .886} 53.6 \\
    Deepseekcoder-V2 & 236B  & \cellcolor[rgb]{ .58,  .702,  .859} 66.6 & \cellcolor[rgb]{ .584,  .706,  .859} 66.2 & \cellcolor[rgb]{ .6,  .718,  .863} 63.4 & \cellcolor[rgb]{ .573,  .698,  .855} 68.0 & \cellcolor[rgb]{ .576,  .698,  .855} 67.6 & \cellcolor[rgb]{ .588,  .71,  .859} 65.4 & \cellcolor[rgb]{ .592,  .71,  .863} 64.8 & \cellcolor[rgb]{ .6,  .718,  .863} 63.6 & \cellcolor[rgb]{ .604,  .718,  .867} 63.0 & \cellcolor[rgb]{ .576,  .698,  .855} 67.4 & \cellcolor[rgb]{ .58,  .702,  .859} 66.8 & \cellcolor[rgb]{ .604,  .718,  .867} 63.0 & \cellcolor[rgb]{ .608,  .722,  .867} 62.2 & \cellcolor[rgb]{ .592,  .71,  .859} 65.2 & \cellcolor[rgb]{ .588,  .706,  .859} 65.8 & \cellcolor[rgb]{ .604,  .718,  .867} 63.2 & \cellcolor[rgb]{ .631,  .737,  .875} 58.8 & \cellcolor[rgb]{ .573,  .698,  .855} 67.8 & \cellcolor[rgb]{ .584,  .702,  .859} 66.4 \\
    Qwen2-Instruct & 72B   & \cellcolor[rgb]{ .678,  .773,  .89} 51.2 & \cellcolor[rgb]{ .686,  .776,  .894} 50.2 & \cellcolor[rgb]{ .675,  .769,  .89} 51.6 & \cellcolor[rgb]{ .663,  .761,  .886} 53.6 & \cellcolor[rgb]{ .761,  .831,  .918} 38.2 & \cellcolor[rgb]{ .675,  .769,  .89} 52.0 & \cellcolor[rgb]{ .678,  .773,  .89} 51.0 & \cellcolor[rgb]{ .694,  .78,  .894} 49.0 & \cellcolor[rgb]{ .714,  .796,  .902} 45.8 & \cellcolor[rgb]{ .682,  .773,  .89} 50.8 & \cellcolor[rgb]{ .678,  .773,  .89} 51.2 & \cellcolor[rgb]{ .718,  .8,  .906} 45.0 & \cellcolor[rgb]{ .706,  .792,  .902} 46.8 & \cellcolor[rgb]{ .682,  .773,  .89} 50.8 & \cellcolor[rgb]{ .678,  .773,  .89} 51.0 & \cellcolor[rgb]{ .678,  .773,  .89} 51.0 & \cellcolor[rgb]{ .714,  .796,  .902} 45.6 & \cellcolor[rgb]{ .682,  .776,  .894} 50.4 & \cellcolor[rgb]{ .667,  .765,  .886} 53.2 \\
    CodeLlama-Python & 34B   & \cellcolor[rgb]{ .741,  .816,  .914} 41.4 & \cellcolor[rgb]{ .718,  .8,  .906} 44.8 & \cellcolor[rgb]{ .714,  .796,  .902} 45.6 & \cellcolor[rgb]{ .737,  .816,  .91} 41.8 & \cellcolor[rgb]{ .741,  .816,  .914} 41.4 & \cellcolor[rgb]{ .718,  .8,  .902} 45.4 & \cellcolor[rgb]{ .718,  .8,  .906} 45.2 & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 & \cellcolor[rgb]{ .725,  .808,  .906} 43.6 & \cellcolor[rgb]{ .725,  .804,  .906} 43.8 & \cellcolor[rgb]{ .725,  .804,  .906} 43.8 & \cellcolor[rgb]{ .733,  .812,  .91} 42.4 & \cellcolor[rgb]{ .757,  .827,  .918} 38.6 & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 & \cellcolor[rgb]{ .71,  .792,  .902} 46.6 & \cellcolor[rgb]{ .725,  .804,  .906} 43.8 & \cellcolor[rgb]{ .737,  .812,  .91} 42.0 & \cellcolor[rgb]{ .722,  .804,  .906} 44.4 & \cellcolor[rgb]{ .718,  .8,  .906} 44.8 \\
    CodeLlama-Instruct & 34B   & \cellcolor[rgb]{ .722,  .804,  .906} 44.4 & \cellcolor[rgb]{ .71,  .796,  .902} 46.2 & \cellcolor[rgb]{ .714,  .796,  .902} 45.8 & \cellcolor[rgb]{ .706,  .792,  .902} 46.8 & \cellcolor[rgb]{ .745,  .82,  .914} 40.6 & \cellcolor[rgb]{ .702,  .788,  .898} 47.4 & \cellcolor[rgb]{ .714,  .796,  .902} 45.6 & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 & \cellcolor[rgb]{ .725,  .804,  .906} 44.0 & \cellcolor[rgb]{ .718,  .8,  .906} 44.8 & \cellcolor[rgb]{ .725,  .804,  .906} 44.0 & \cellcolor[rgb]{ .749,  .824,  .914} 40.2 & \cellcolor[rgb]{ .761,  .831,  .918} 38.2 & \cellcolor[rgb]{ .722,  .804,  .906} 44.2 & \cellcolor[rgb]{ .71,  .792,  .902} 46.4 & \cellcolor[rgb]{ .725,  .804,  .906} 43.8 & \cellcolor[rgb]{ .745,  .82,  .914} 40.6 & \cellcolor[rgb]{ .718,  .8,  .906} 45.2 & \cellcolor[rgb]{ .718,  .8,  .906} 45.0 \\
    CodeLlama & 34B   & \cellcolor[rgb]{ .722,  .8,  .906} 44.6 & \cellcolor[rgb]{ .702,  .788,  .898} 47.8 & \cellcolor[rgb]{ .722,  .804,  .906} 44.2 & \cellcolor[rgb]{ .718,  .8,  .906} 45.2 & \cellcolor[rgb]{ .761,  .831,  .918} 38.4 & \cellcolor[rgb]{ .706,  .792,  .898} 47.0 & \cellcolor[rgb]{ .714,  .796,  .902} 45.8 & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 & \cellcolor[rgb]{ .725,  .804,  .906} 43.8 & \cellcolor[rgb]{ .71,  .792,  .902} 46.4 & \cellcolor[rgb]{ .71,  .792,  .902} 46.4 & \cellcolor[rgb]{ .757,  .827,  .918} 38.8 & \cellcolor[rgb]{ .761,  .831,  .918} 38.4 & \cellcolor[rgb]{ .718,  .8,  .902} 45.4 & \cellcolor[rgb]{ .706,  .788,  .898} 47.2 & \cellcolor[rgb]{ .702,  .788,  .898} 47.4 & \cellcolor[rgb]{ .725,  .804,  .906} 43.8 & \cellcolor[rgb]{ .702,  .788,  .898} 47.6 & \cellcolor[rgb]{ .702,  .788,  .898} 47.4 \\
    WizardCoder-V1.1 & 33B   & \cellcolor[rgb]{ .706,  .792,  .898} 47.0 & \cellcolor[rgb]{ .706,  .792,  .902} 46.8 & \cellcolor[rgb]{ .714,  .796,  .902} 45.8 & \cellcolor[rgb]{ .722,  .804,  .906} 44.2 & \cellcolor[rgb]{ .682,  .773,  .89} 50.8 & \cellcolor[rgb]{ .686,  .776,  .894} 50.0 & \cellcolor[rgb]{ .706,  .792,  .898} 47.0 & \cellcolor[rgb]{ .714,  .796,  .902} 46.0 & \cellcolor[rgb]{ .718,  .8,  .906} 45.2 & \cellcolor[rgb]{ .678,  .773,  .89} 51.4 & \cellcolor[rgb]{ .69,  .78,  .894} 49.6 & \cellcolor[rgb]{ .725,  .804,  .906} 44.0 & \cellcolor[rgb]{ .733,  .812,  .91} 42.4 & \cellcolor[rgb]{ .698,  .784,  .898} 48.2 & \cellcolor[rgb]{ .702,  .788,  .898} 47.8 & \cellcolor[rgb]{ .718,  .8,  .906} 45.0 & \cellcolor[rgb]{ .722,  .804,  .906} 44.4 & \cellcolor[rgb]{ .698,  .788,  .898} 48.0 & \cellcolor[rgb]{ .686,  .776,  .894} 49.8 \\
    Deepseekcoder-instruct & 33B   & \cellcolor[rgb]{ .675,  .769,  .89} 52.0 & \cellcolor[rgb]{ .678,  .773,  .89} 51.4 & \cellcolor[rgb]{ .694,  .78,  .894} 49.0 & \cellcolor[rgb]{ .694,  .784,  .898} 48.8 & \cellcolor[rgb]{ .667,  .765,  .886} 53.2 & \cellcolor[rgb]{ .655,  .753,  .882} 55.0 & \cellcolor[rgb]{ .682,  .776,  .894} 50.4 & \cellcolor[rgb]{ .682,  .776,  .894} 50.4 & \cellcolor[rgb]{ .686,  .776,  .894} 50.0 & \cellcolor[rgb]{ .667,  .765,  .886} 53.0 & \cellcolor[rgb]{ .675,  .769,  .89} 52.2 & \cellcolor[rgb]{ .698,  .784,  .898} 48.2 & \cellcolor[rgb]{ .71,  .792,  .902} 46.6 & \cellcolor[rgb]{ .671,  .765,  .886} 52.8 & \cellcolor[rgb]{ .682,  .776,  .894} 50.6 & \cellcolor[rgb]{ .698,  .788,  .898} 48.0 & \cellcolor[rgb]{ .69,  .78,  .894} 49.4 & \cellcolor[rgb]{ .671,  .765,  .886} 52.8 & \cellcolor[rgb]{ .663,  .761,  .886} 53.6 \\
    DeepseekCoder-base & 33B   & \cellcolor[rgb]{ .698,  .784,  .898} 48.2 & \cellcolor[rgb]{ .686,  .776,  .894} 50.0 & \cellcolor[rgb]{ .714,  .796,  .902} 46.0 & \cellcolor[rgb]{ .694,  .784,  .898} 48.6 & \cellcolor[rgb]{ .69,  .78,  .894} 49.2 & \cellcolor[rgb]{ .678,  .773,  .89} 51.4 & \cellcolor[rgb]{ .706,  .792,  .902} 46.8 & \cellcolor[rgb]{ .698,  .788,  .898} 48.0 & \cellcolor[rgb]{ .698,  .784,  .898} 48.4 & \cellcolor[rgb]{ .675,  .769,  .89} 52.0 & \cellcolor[rgb]{ .686,  .776,  .894} 49.8 & \cellcolor[rgb]{ .718,  .8,  .906} 45.2 & \cellcolor[rgb]{ .71,  .792,  .902} 46.4 & \cellcolor[rgb]{ .694,  .78,  .894} 49.0 & \cellcolor[rgb]{ .71,  .796,  .902} 46.2 & \cellcolor[rgb]{ .702,  .788,  .898} 47.6 & \cellcolor[rgb]{ .714,  .796,  .902} 46.0 & \cellcolor[rgb]{ .69,  .78,  .894} 49.2 & \cellcolor[rgb]{ .678,  .773,  .89} 51.2 \\
    Starcoder2 & 15B   & \cellcolor[rgb]{ .714,  .796,  .902} 46.0 & \cellcolor[rgb]{ .702,  .788,  .898} 47.4 & \cellcolor[rgb]{ .706,  .788,  .898} 47.2 & \cellcolor[rgb]{ .694,  .78,  .894} 49.0 & \cellcolor[rgb]{ .698,  .784,  .898} 48.4 & \cellcolor[rgb]{ .686,  .776,  .894} 50.0 & \cellcolor[rgb]{ .69,  .78,  .894} 49.2 & \cellcolor[rgb]{ .718,  .8,  .906} 44.8 & \cellcolor[rgb]{ .69,  .78,  .894} 49.4 & \cellcolor[rgb]{ .698,  .784,  .898} 48.4 & \cellcolor[rgb]{ .698,  .784,  .898} 48.4 & \cellcolor[rgb]{ .706,  .788,  .898} 47.2 & \cellcolor[rgb]{ .718,  .8,  .906} 45.0 & \cellcolor[rgb]{ .678,  .773,  .89} 51.0 & \cellcolor[rgb]{ .694,  .784,  .898} 48.8 & \cellcolor[rgb]{ .718,  .8,  .906} 45.2 & \cellcolor[rgb]{ .714,  .796,  .902} 45.8 & \cellcolor[rgb]{ .69,  .78,  .894} 49.6 & \cellcolor[rgb]{ .694,  .784,  .898} 48.6 \\
    WizardCoder-V1.0 & 15B   & \cellcolor[rgb]{ .843,  .89,  .949} 25.2 & \cellcolor[rgb]{ .812,  .867,  .937} 30.0 & \cellcolor[rgb]{ .808,  .867,  .937} 30.6 & \cellcolor[rgb]{ .792,  .855,  .929} 33.2 & \cellcolor[rgb]{ .835,  .882,  .945} 26.8 & \cellcolor[rgb]{ .792,  .851,  .929} 33.6 & \cellcolor[rgb]{ .812,  .867,  .937} 30.2 & \cellcolor[rgb]{ .812,  .867,  .937} 30.2 & \cellcolor[rgb]{ .808,  .863,  .933} 31.0 & \cellcolor[rgb]{ .796,  .855,  .929} 33.0 & \cellcolor[rgb]{ .788,  .851,  .929} 34.0 & \cellcolor[rgb]{ .804,  .859,  .933} 31.6 & \cellcolor[rgb]{ .816,  .871,  .937} 29.6 & \cellcolor[rgb]{ .796,  .855,  .929} 32.8 & \cellcolor[rgb]{ .804,  .863,  .933} 31.2 & \cellcolor[rgb]{ .804,  .863,  .933} 31.2 & \cellcolor[rgb]{ .816,  .867,  .937} 29.8 & \cellcolor[rgb]{ .788,  .847,  .929} 34.2 & \cellcolor[rgb]{ .788,  .851,  .929} 34.0 \\
    Starcoder & 15B   & \cellcolor[rgb]{ .875,  .91,  .957} 20.4 & \cellcolor[rgb]{ .804,  .859,  .933} 31.6 & \cellcolor[rgb]{ .8,  .859,  .933} 31.8 & \cellcolor[rgb]{ .808,  .863,  .933} 31.0 & \cellcolor[rgb]{ .886,  .922,  .961} 18.4 & \cellcolor[rgb]{ .792,  .851,  .929} 33.4 & \cellcolor[rgb]{ .8,  .859,  .933} 32.2 & \cellcolor[rgb]{ .8,  .859,  .933} 31.8 & \cellcolor[rgb]{ .816,  .867,  .937} 29.8 & \cellcolor[rgb]{ .796,  .855,  .929} 32.6 & \cellcolor[rgb]{ .796,  .855,  .929} 32.6 & \cellcolor[rgb]{ .812,  .867,  .937} 30.0 & \cellcolor[rgb]{ .82,  .871,  .937} 29.2 & \cellcolor[rgb]{ .792,  .851,  .929} 33.4 & \cellcolor[rgb]{ .796,  .855,  .929} 32.6 & \cellcolor[rgb]{ .812,  .867,  .937} 30.0 & \cellcolor[rgb]{ .812,  .867,  .937} 30.2 & \cellcolor[rgb]{ .796,  .855,  .929} 33.0 & \cellcolor[rgb]{ .796,  .855,  .929} 33.0 \\
    phi-3-instruct & 14B   & \cellcolor[rgb]{ .788,  .847,  .929} 34.2 & \cellcolor[rgb]{ .765,  .831,  .922} 37.6 & \cellcolor[rgb]{ .757,  .827,  .918} 39.0 & \cellcolor[rgb]{ .808,  .863,  .933} 31.0 & \cellcolor[rgb]{ .788,  .847,  .929} 34.2 & \cellcolor[rgb]{ .741,  .816,  .914} 41.6 & \cellcolor[rgb]{ .741,  .816,  .914} 41.2 & \cellcolor[rgb]{ .784,  .847,  .929} 34.4 & \cellcolor[rgb]{ .776,  .843,  .925} 35.8 & \cellcolor[rgb]{ .765,  .831,  .922} 37.8 & \cellcolor[rgb]{ .733,  .812,  .91} 42.4 & \cellcolor[rgb]{ .773,  .839,  .922} 36.6 & \cellcolor[rgb]{ .847,  .89,  .949} 24.6 & \cellcolor[rgb]{ .737,  .812,  .91} 42.2 & \cellcolor[rgb]{ .765,  .835,  .922} 37.4 & \cellcolor[rgb]{ .773,  .839,  .922} 36.2 & \cellcolor[rgb]{ .769,  .835,  .922} 37.2 & \cellcolor[rgb]{ .741,  .816,  .914} 41.4 & \cellcolor[rgb]{ .729,  .808,  .91} 43.0 \\
    Llama-3-Instruct & 8B    & \cellcolor[rgb]{ .8,  .859,  .933} 32.0 & \cellcolor[rgb]{ .808,  .863,  .933} 30.8 & \cellcolor[rgb]{ .804,  .863,  .933} 31.2 & \cellcolor[rgb]{ .804,  .863,  .933} 31.4 & \cellcolor[rgb]{ .843,  .89,  .949} 25.0 & \cellcolor[rgb]{ .78,  .843,  .925} 35.0 & \cellcolor[rgb]{ .804,  .863,  .933} 31.4 & \cellcolor[rgb]{ .788,  .851,  .929} 34.0 & \cellcolor[rgb]{ .816,  .871,  .937} 29.6 & \cellcolor[rgb]{ .831,  .882,  .945} 27.0 & \cellcolor[rgb]{ .792,  .851,  .929} 33.6 & \cellcolor[rgb]{ .831,  .878,  .945} 27.2 & \cellcolor[rgb]{ .827,  .878,  .941} 28.0 & \cellcolor[rgb]{ .8,  .859,  .933} 31.8 & \cellcolor[rgb]{ .784,  .847,  .929} 34.4 & \cellcolor[rgb]{ .788,  .851,  .929} 33.8 & \cellcolor[rgb]{ .8,  .859,  .933} 32.0 & \cellcolor[rgb]{ .773,  .839,  .922} 36.4 & \cellcolor[rgb]{ .788,  .851,  .929} 33.8 \\
    CodeQwen1.5-Chat & 7B    & \cellcolor[rgb]{ .765,  .831,  .922} 37.8 & \cellcolor[rgb]{ .749,  .824,  .914} 40.2 & \cellcolor[rgb]{ .749,  .824,  .914} 40.2 & \cellcolor[rgb]{ .745,  .82,  .914} 40.6 & \cellcolor[rgb]{ .78,  .843,  .925} 35.4 & \cellcolor[rgb]{ .725,  .808,  .906} 43.6 & \cellcolor[rgb]{ .733,  .812,  .91} 42.6 & \cellcolor[rgb]{ .749,  .82,  .914} 40.4 & \cellcolor[rgb]{ .753,  .824,  .918} 39.6 & \cellcolor[rgb]{ .729,  .808,  .91} 43.0 & \cellcolor[rgb]{ .741,  .816,  .914} 41.4 & \cellcolor[rgb]{ .761,  .831,  .918} 38.2 & \cellcolor[rgb]{ .757,  .827,  .918} 39.0 & \cellcolor[rgb]{ .722,  .8,  .906} 44.6 & \cellcolor[rgb]{ .737,  .812,  .91} 42.0 & \cellcolor[rgb]{ .78,  .843,  .925} 35.0 & \cellcolor[rgb]{ .761,  .831,  .918} 38.2 & \cellcolor[rgb]{ .725,  .804,  .906} 43.8 & \cellcolor[rgb]{ .737,  .812,  .91} 42.2 \\
    CodeLlama-Instruct & 7B    & \cellcolor[rgb]{ .8,  .859,  .933} 32.2 & \cellcolor[rgb]{ .776,  .843,  .925} 35.6 & \cellcolor[rgb]{ .784,  .847,  .929} 34.4 & \cellcolor[rgb]{ .78,  .843,  .925} 35.0 & \cellcolor[rgb]{ .847,  .894,  .949} 24.4 & \cellcolor[rgb]{ .761,  .831,  .918} 38.2 & \cellcolor[rgb]{ .78,  .843,  .925} 35.2 & \cellcolor[rgb]{ .8,  .859,  .933} 32.2 & \cellcolor[rgb]{ .788,  .847,  .929} 34.2 & \cellcolor[rgb]{ .776,  .839,  .925} 36.0 & \cellcolor[rgb]{ .78,  .843,  .925} 35.4 & \cellcolor[rgb]{ .8,  .859,  .933} 32.0 & \cellcolor[rgb]{ .816,  .871,  .937} 29.6 & \cellcolor[rgb]{ .769,  .835,  .922} 37.0 & \cellcolor[rgb]{ .765,  .835,  .922} 37.4 & \cellcolor[rgb]{ .796,  .855,  .929} 33.0 & \cellcolor[rgb]{ .796,  .855,  .929} 33.0 & \cellcolor[rgb]{ .784,  .847,  .925} 34.6 & \cellcolor[rgb]{ .757,  .827,  .918} 38.8 \\
    CodeLlama-hf & 7B    & \cellcolor[rgb]{ .796,  .855,  .929} 32.6 & \cellcolor[rgb]{ .784,  .847,  .929} 34.4 & \cellcolor[rgb]{ .788,  .851,  .929} 33.8 & \cellcolor[rgb]{ .792,  .851,  .929} 33.4 & \cellcolor[rgb]{ .824,  .875,  .941} 28.4 & \cellcolor[rgb]{ .761,  .831,  .922} 38.0 & \cellcolor[rgb]{ .78,  .843,  .925} 35.2 & \cellcolor[rgb]{ .784,  .847,  .929} 34.4 & \cellcolor[rgb]{ .78,  .843,  .925} 35.2 & \cellcolor[rgb]{ .761,  .831,  .922} 38.0 & \cellcolor[rgb]{ .784,  .847,  .929} 34.4 & \cellcolor[rgb]{ .796,  .855,  .929} 32.6 & \cellcolor[rgb]{ .808,  .863,  .933} 30.8 & \cellcolor[rgb]{ .784,  .847,  .925} 34.8 & \cellcolor[rgb]{ .769,  .835,  .922} 36.8 & \cellcolor[rgb]{ .792,  .851,  .929} 33.4 & \cellcolor[rgb]{ .808,  .863,  .933} 31.0 & \cellcolor[rgb]{ .78,  .843,  .925} 35.0 & \cellcolor[rgb]{ .761,  .831,  .918} 38.2 \\
    Deepseekcoder-instruct & 6.7B  & \cellcolor[rgb]{ .784,  .847,  .925} 34.8 & \cellcolor[rgb]{ .737,  .816,  .91} 41.8 & \cellcolor[rgb]{ .749,  .82,  .914} 40.4 & \cellcolor[rgb]{ .753,  .824,  .918} 39.4 & \cellcolor[rgb]{ .796,  .855,  .929} 32.8 & \cellcolor[rgb]{ .702,  .788,  .898} 47.6 & \cellcolor[rgb]{ .733,  .812,  .91} 42.6 & \cellcolor[rgb]{ .757,  .827,  .918} 38.8 & \cellcolor[rgb]{ .737,  .812,  .91} 42.0 & \cellcolor[rgb]{ .725,  .804,  .906} 43.8 & \cellcolor[rgb]{ .725,  .808,  .906} 43.6 & \cellcolor[rgb]{ .745,  .82,  .914} 40.8 & \cellcolor[rgb]{ .757,  .827,  .918} 39.2 & \cellcolor[rgb]{ .729,  .808,  .91} 43.2 & \cellcolor[rgb]{ .737,  .816,  .91} 41.8 & \cellcolor[rgb]{ .745,  .82,  .914} 40.6 & \cellcolor[rgb]{ .765,  .831,  .922} 37.8 & \cellcolor[rgb]{ .729,  .808,  .91} 43.2 & \cellcolor[rgb]{ .725,  .804,  .906} 44.0 \\
    Deepseekcoder-base & 6.7B  & \cellcolor[rgb]{ .741,  .816,  .914} 41.2 & \cellcolor[rgb]{ .71,  .796,  .902} 46.2 & \cellcolor[rgb]{ .729,  .808,  .91} 43.2 & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 & \cellcolor[rgb]{ .733,  .812,  .91} 42.6 & \cellcolor[rgb]{ .718,  .8,  .906} 44.8 & \cellcolor[rgb]{ .714,  .796,  .902} 46.0 & \cellcolor[rgb]{ .745,  .82,  .914} 41.0 & \cellcolor[rgb]{ .749,  .82,  .914} 40.4 & \cellcolor[rgb]{ .737,  .816,  .91} 41.8 & \cellcolor[rgb]{ .718,  .8,  .906} 44.8 & \cellcolor[rgb]{ .733,  .812,  .91} 42.8 & \cellcolor[rgb]{ .729,  .808,  .91} 43.0 & \cellcolor[rgb]{ .733,  .812,  .91} 42.6 & \cellcolor[rgb]{ .737,  .812,  .91} 42.0 & \cellcolor[rgb]{ .729,  .808,  .91} 43.2 & \cellcolor[rgb]{ .745,  .82,  .914} 40.6 & \cellcolor[rgb]{ .702,  .788,  .898} 47.6 & \cellcolor[rgb]{ .718,  .8,  .902} 45.4 \\
    CodeGen-multi & 6B    & \cellcolor[rgb]{ .867,  .906,  .957} 21.4 & \cellcolor[rgb]{ .855,  .898,  .949} 23.6 & \cellcolor[rgb]{ .843,  .89,  .949} 25.0 & \cellcolor[rgb]{ .835,  .882,  .945} 26.4 & \cellcolor[rgb]{ .867,  .906,  .957} 21.6 & \cellcolor[rgb]{ .859,  .902,  .953} 22.8 & \cellcolor[rgb]{ .859,  .902,  .953} 22.8 & \cellcolor[rgb]{ .851,  .894,  .949} 23.8 & \cellcolor[rgb]{ .875,  .91,  .957} 20.4 & \cellcolor[rgb]{ .843,  .89,  .949} 25.2 & \cellcolor[rgb]{ .847,  .89,  .949} 24.8 & \cellcolor[rgb]{ .855,  .898,  .953} 23.4 & \cellcolor[rgb]{ .89,  .922,  .965} 17.8 & \cellcolor[rgb]{ .851,  .894,  .949} 24.0 & \cellcolor[rgb]{ .843,  .89,  .949} 25.2 & \cellcolor[rgb]{ .863,  .902,  .953} 22.0 & \cellcolor[rgb]{ .863,  .902,  .953} 22.2 & \cellcolor[rgb]{ .843,  .89,  .949} 25.0 & \cellcolor[rgb]{ .867,  .906,  .957} 21.4 \\
    phi-1\_5 & 1.3B  & \cellcolor[rgb]{ .902,  .929,  .969} 16.0 & \cellcolor[rgb]{ .839,  .886,  .945} 26.0 & \cellcolor[rgb]{ .847,  .89,  .949} 24.8 & \cellcolor[rgb]{ .859,  .902,  .953} 22.6 & \cellcolor[rgb]{ .902,  .933,  .969} 15.8 & \cellcolor[rgb]{ .859,  .898,  .953} 23.0 & \cellcolor[rgb]{ .855,  .898,  .949} 23.6 & \cellcolor[rgb]{ .871,  .906,  .957} 21.2 & \cellcolor[rgb]{ .863,  .902,  .953} 22.0 & \cellcolor[rgb]{ .863,  .902,  .953} 22.2 & \cellcolor[rgb]{ .839,  .886,  .945} 25.6 & \cellcolor[rgb]{ .867,  .906,  .953} 21.8 & \cellcolor[rgb]{ .898,  .925,  .965} 16.8 & \cellcolor[rgb]{ .878,  .914,  .961} 19.6 & \cellcolor[rgb]{ .863,  .902,  .953} 22.0 & \cellcolor[rgb]{ .867,  .906,  .957} 21.6 & \cellcolor[rgb]{ .89,  .922,  .965} 17.6 & \cellcolor[rgb]{ .839,  .886,  .945} 25.6 & \cellcolor[rgb]{ .843,  .89,  .949} 25.2 \\
    phi-1 & 1.3B  & \cellcolor[rgb]{ .965,  .976,  .988} 5.8 & \cellcolor[rgb]{ .945,  .961,  .984} 9.0 & \cellcolor[rgb]{ .922,  .945,  .973} 13.2 & \cellcolor[rgb]{ .91,  .937,  .969} 14.8 & \cellcolor[rgb]{ .973,  .98,  .992} 4.6 & \cellcolor[rgb]{ .871,  .91,  .957} 20.8 & \cellcolor[rgb]{ .882,  .918,  .961} 19.2 & \cellcolor[rgb]{ .902,  .933,  .969} 15.8 & \cellcolor[rgb]{ .906,  .933,  .969} 15.6 & \cellcolor[rgb]{ .886,  .918,  .961} 18.6 & \cellcolor[rgb]{ .863,  .902,  .953} 22.4 & \cellcolor[rgb]{ .89,  .922,  .965} 17.6 & \cellcolor[rgb]{ .937,  .957,  .98} 10.4 & \cellcolor[rgb]{ .89,  .922,  .965} 18.0 & \cellcolor[rgb]{ .898,  .929,  .965} 16.4 & \cellcolor[rgb]{ .933,  .953,  .976} 11.0 & \cellcolor[rgb]{ .898,  .929,  .965} 16.4 & \cellcolor[rgb]{ .882,  .918,  .961} 19.2 & \cellcolor[rgb]{ .882,  .918,  .961} 19.0 \\
    \midrule
    Average &       & 40.3  & 42.4  & 42.3  & 42.6  & 37.9  & 45.1  & 43.1  & 41.6  & 41.3  & 43.8  & 44.2  & 40.4  & 38.3  & 43.5  & 43.4  & 41.5  & 40.1  & 44.6  & 44.6 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%
